Still Manual? Automated Linter Configuration via DSL-Based LLM Compilation of Coding Standards

Coding standards are essential for maintaining consistent and high-quality code across teams and projects. Linters help developers enforce these standards by detecting code violations. However, manual linter configuration is complex and expertise-intensive, and the diversity and evolution of programming languages, coding standards, and linters lead to repetitive and maintenance-intensive configuration work. To reduce manual effort, we propose LintCFG, a domain-specific language (DSL)-driven, LLM-based compilation approach to automate linter configuration generation for coding standards, independent of programming languages, coding standards, and linters. Inspired by compiler design, we first design a DSL to express coding rules in a tool-agnostic, structured, readable, and precise manner. Then, we build linter configurations into DSL configuration instructions. For a given natural language coding standard, the compilation process parses it into DSL coding standards, matches them with the DSL configuration instructions to set configuration names, option names and values, verifies consistency between the standards and configurations, and finally generates linter-specific configurations. Experiments with Checkstyle for Java coding standard show that our approach achieves over 90% precision and recall in DSL representation, with accuracy, precision, recall, and F1-scores close to 70% (with some exceeding 70%) in fine-grained linter configuration generation. Notably, our approach outperforms baselines by over 100% in precision. A user study further shows that our approach improves developers' efficiency in configuring linters for coding standards. Finally, we demonstrate the generality of the approach by generating ESLint configurations for JavaScript coding standards, showcasing its broad applicability across other programming languages, coding standards, and linters.

==> dsl_stat.tex <==

\begin{table}[h]
\label{tab:dsl}
\centering
\scalebox{0.85}{
\begin{tabular}{clllllll}
\multicolumn{1}{c}{\cellcolor[gray]{0.9}}&
\multicolumn{1}{|c|}{\cellcolor[gray]{0.9}Name}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}\#Rule}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}\#DSL}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Acc(\%)}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}P(\%)}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}R(\%)}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}F(\%)}\\ \hline


\multirow{2}{*}{Coding Standard}&
\multicolumn{1}{|c|}{Google Java Style Guide}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}\\
\cline{2-8}&
\multicolumn{1}{|c|}{Google JavaScript Style Guide}&
\multicolumn{1}{c}{108}&
\multicolumn{1}{c}{394}&
\multicolumn{1}{c}{74.1}&
\multicolumn{1}{c}{90.6}&
\multicolumn{1}{c}{99.4}&
\multicolumn{1}{c}{94.8}\\ \hline


\multirow{2}{*}{Tool}&
\multicolumn{1}{|c|}{Checkstyle}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}&
\multicolumn{1}{c}{1}\\
\cline{2-8}&
\multicolumn{1}{|c|}{ESLint}&
\multicolumn{1}{c}{166}&
\multicolumn{1}{c}{528(basic 304)}&
\multicolumn{1}{c}{78.3}&
\multicolumn{1}{c}{87.4}&
\multicolumn{1}{c}{99.4}&
\multicolumn{1}{c}{93.0}\\ \hline

\end{tabular}
}

\end{table}


==> evaluation_improvement.tex <==
\noindent \textbf{Note:}   Underlined values indicate the best performance among the baselines. Bold values represent the best performance across all methods. "Improvement" indicates the minimum improvement over the baselines. For baselines that cannot be run due to token limits, results are marked with '-'.


\begin{table}[h]
\scriptsize\caption{Results of Generating Checkstyle Configuration for Google Java Style Guide.}
  \label{tab:checkstyle_result_table}
  \vspace{-0.1cm}
\centering
\scalebox{0.8}{
\begin{tabular}{|c|llllllllllll|}
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{|c|}{Rule Name} &
\multicolumn{4}{|c|}{Option Name} &
\multicolumn{4}{|c|}{Option Value} \\
\cline{2-13} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} \\ \hline

\multicolumn{1}{|c|}{closed book}&\multicolumn{1}{|c|}{38.2}&\multicolumn{1}{|c|}{\underline{39.4}}&\multicolumn{1}{|c|}{58.6}&\multicolumn{1}{|c|}{\underline{47.1}}&\multicolumn{1}{|c|}{20.6}&\multicolumn{1}{|c|}{24.0}&\multicolumn{1}{|c|}{35.7}&\multicolumn{1}{|c|}{28.7}&\multicolumn{1}{|c|}{33.8}&\multicolumn{1}{|c|}{\underline{28.8}}&\multicolumn{1}{|c|}{42.9}&\multicolumn{1}{|c|}{\underline{34.5}}\\ \hline

\multicolumn{1}{|c|}{name}&\multicolumn{1}{|c|}{42.6}&\multicolumn{1}{|c|}{17.1}&\multicolumn{1}{|c|}{81.2}&\multicolumn{1}{|c|}{28.3}&\multicolumn{1}{|c|}{23.5}&\multicolumn{1}{|c|}{11.3}&\multicolumn{1}{|c|}{53.6}&\multicolumn{1}{|c|}{18.7}&\multicolumn{1}{|c|}{33.8}&\multicolumn{1}{|c|}{12.5}&\multicolumn{1}{|c|}{59.4}&\multicolumn{1}{|c|}{20.7}\\ \hline

\multicolumn{1}{|c|}{name\_desc}&\multicolumn{1}{|c|}{44.1}&\multicolumn{1}{|c|}{25.7}&\multicolumn{1}{|c|}{80.9}&\multicolumn{1}{|c|}{39.0}&\multicolumn{1}{|c|}{29.4}&\multicolumn{1}{|c|}{20.1}&\multicolumn{1}{|c|}{63.2}&\multicolumn{1}{|c|}{30.5}&\multicolumn{1}{|c|}{30.9}&\multicolumn{1}{|c|}{17.3}&\multicolumn{1}{|c|}{54.4}&\multicolumn{1}{|c|}{26.2}\\ \hline

\multicolumn{1}{|c|}{name\_desc\_opt}&\multicolumn{1}{|c|}{\underline{51.5}}&\multicolumn{1}{|c|}{23.4}&\multicolumn{1}{|c|}{\textbf{\underline{84.1}}}&\multicolumn{1}{|c|}{36.6}&\multicolumn{1}{|c|}{\underline{51.5}}&\multicolumn{1}{|c|}{23.0}&\multicolumn{1}{|c|}{\textbf{\underline{82.6}}}&\multicolumn{1}{|c|}{36.0}&\multicolumn{1}{|c|}{\underline{39.7}}&\multicolumn{1}{|c|}{17.7}&\multicolumn{1}{|c|}{\underline{63.8}}&\multicolumn{1}{|c|}{27.8}\\ \hline

\multicolumn{1}{|c|}{name\_desc (RAG)}&\multicolumn{1}{|c|}{16.2}&\multicolumn{1}{|c|}{23.5}&\multicolumn{1}{|c|}{77.6}&\multicolumn{1}{|c|}{36.1}&\multicolumn{1}{|c|}{14.7}&\multicolumn{1}{|c|}{20.4}&\multicolumn{1}{|c|}{67.2}&\multicolumn{1}{|c|}{31.2}&\multicolumn{1}{|c|}{13.2}&\multicolumn{1}{|c|}{16.3}&\multicolumn{1}{|c|}{53.7}&\multicolumn{1}{|c|}{25.0}\\ \hline

\multicolumn{1}{|c|}{name\_desc\_opt (RAG)}&\multicolumn{1}{|c|}{25.0}&\multicolumn{1}{|c|}{31.8}&\multicolumn{1}{|c|}{79.4}&\multicolumn{1}{|c|}{45.4}&\multicolumn{1}{|c|}{25.0}&\multicolumn{1}{|c|}{\underline{31.8}}&\multicolumn{1}{|c|}{79.4}&\multicolumn{1}{|c|}{\underline{45.4}}&\multicolumn{1}{|c|}{13.2}&\multicolumn{1}{|c|}{17.6}&\multicolumn{1}{|c|}{44.1}&\multicolumn{1}{|c|}{25.2}\\ \hline

\multicolumn{1}{|c|}{\textbf{Our Method}}&\multicolumn{1}{|c|}{\textbf{81.2}}&\multicolumn{1}{|c|}{\textbf{92.1}}&\multicolumn{1}{|c|}{\textbf{\underline{84.1}}}&\multicolumn{1}{|c|}{\textbf{87.9}}&\multicolumn{1}{|c|}{\textbf{78.3}}&\multicolumn{1}{|c|}{\textbf{84.1}}&\multicolumn{1}{|c|}{76.8}&\multicolumn{1}{|c|}{\textbf{80.3}}&\multicolumn{1}{|c|}{\textbf{76.8}}&\multicolumn{1}{|c|}{\textbf{76.2}}&\multicolumn{1}{|c|}{\textbf{69.6}}&\multicolumn{1}{|c|}{\textbf{72.7}}\\ \hline

\multicolumn{1}{|c|}{Improvement}&\multicolumn{1}{|c|}{57.7}&\multicolumn{1}{|c|}{133.8}&\multicolumn{1}{|c|}{0.0}&\multicolumn{1}{|c|}{86.6}&\multicolumn{1}{|c|}{52.0}&\multicolumn{1}{|c|}{164.5}&\multicolumn{1}{|c|}{-7.0}&\multicolumn{1}{|c|}{76.9}&\multicolumn{1}{|c|}{93.5}&\multicolumn{1}{|c|}{164.6}&\multicolumn{1}{|c|}{9.1}&\multicolumn{1}{|c|}{110.7}\\ \hline


\end{tabular}
}
\vspace{-0.2cm}
\end{table}


\begin{table}[h]
\scriptsize\caption{Results of Generating ESLint Configuration for Google JavaScript Style Guide.}
  \label{tab:ESLint_result_table}
  \vspace{-0.1cm}
\centering
\scalebox{0.8}{
\begin{tabular}{|c|llllllllllll|}
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{|c|}{Rule Name} &
\multicolumn{4}{|c|}{Option Name} &
\multicolumn{4}{|c|}{Option Value} \\
\cline{2-13} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} &
\multicolumn{1}{|c|}{cs\text{-}Acc (\%)} &
\multicolumn{1}{|c|}{P (\%)} &
\multicolumn{1}{|c|}{R (\%)} &
\multicolumn{1}{|c|}{F1(\%)} \\ \hline

\multicolumn{1}{|c|}{closed book}&\multicolumn{1}{|c|}{27.5}&\multicolumn{1}{|c|}{15.5}&\multicolumn{1}{|c|}{65.1}&\multicolumn{1}{|c|}{25.1}&\multicolumn{1}{|c|}{24.8}&\multicolumn{1}{|c|}{11.8}&\multicolumn{1}{|c|}{49.4}&\multicolumn{1}{|c|}{19.0}&\multicolumn{1}{|c|}{24.8}&\multicolumn{1}{|c|}{10.1}&\multicolumn{1}{|c|}{42.2}&\multicolumn{1}{|c|}{16.2}\\ \hline

\multicolumn{1}{|c|}{name}&\multicolumn{1}{|c|}{18.8}&\multicolumn{1}{|c|}{10.5}&\multicolumn{1}{|c|}{83.1}&\multicolumn{1}{|c|}{18.6}&\multicolumn{1}{|c|}{16.1}&\multicolumn{1}{|c|}{7.6}&\multicolumn{1}{|c|}{60.2}&\multicolumn{1}{|c|}{13.5}&\multicolumn{1}{|c|}{16.1}&\multicolumn{1}{|c|}{7.0}&\multicolumn{1}{|c|}{55.4}&\multicolumn{1}{|c|}{12.4}\\ \hline

\multicolumn{1}{|c|}{name\_desc}&\multicolumn{1}{|c|}{\underline{32.2}}&\multicolumn{1}{|c|}{\underline{20.8}}&\multicolumn{1}{|c|}{72.3}&\multicolumn{1}{|c|}{\underline{32.3}}&\multicolumn{1}{|c|}{\underline{28.2}}&\multicolumn{1}{|c|}{\underline{15.3}}&\multicolumn{1}{|c|}{53.0}&\multicolumn{1}{|c|}{\underline{23.7}}&\multicolumn{1}{|c|}{\underline{27.5}}&\multicolumn{1}{|c|}{\underline{14.2}}&\multicolumn{1}{|c|}{49.4}&\multicolumn{1}{|c|}{\underline{22.1}}\\ \hline

\multicolumn{1}{|c|}{name\_desc\_opt}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}&\multicolumn{1}{|c|}{-}\\ \hline

\multicolumn{1}{|c|}{name\_desc (RAG)}&\multicolumn{1}{|c|}{13.4}&\multicolumn{1}{|c|}{9.2}&\multicolumn{1}{|c|}{79.5}&\multicolumn{1}{|c|}{16.5}&\multicolumn{1}{|c|}{10.7}&\multicolumn{1}{|c|}{6.4}&\multicolumn{1}{|c|}{55.4}&\multicolumn{1}{|c|}{11.5}&\multicolumn{1}{|c|}{10.7}&\multicolumn{1}{|c|}{6.0}&\multicolumn{1}{|c|}{51.8}&\multicolumn{1}{|c|}{10.8}\\ \hline

\multicolumn{1}{|c|}{name\_desc\_opt (RAG)}&\multicolumn{1}{|c|}{16.8}&\multicolumn{1}{|c|}{7.8}&\multicolumn{1}{|c|}{\textbf{\underline{85.5}}}&\multicolumn{1}{|c|}{14.4}&\multicolumn{1}{|c|}{13.4}&\multicolumn{1}{|c|}{5.7}&\multicolumn{1}{|c|}{\textbf{\underline{62.7}}}&\multicolumn{1}{|c|}{10.5}&\multicolumn{1}{|c|}{13.4}&\multicolumn{1}{|c|}{5.4}&\multicolumn{1}{|c|}{\underline{59.0}}&\multicolumn{1}{|c|}{9.9}\\ \hline

\multicolumn{1}{|c|}{Our Method}&\multicolumn{1}{|c|}{\textbf{83.1}}&\multicolumn{1}{|c|}{\textbf{83.9}}&\multicolumn{1}{|c|}{67.5}&\multicolumn{1}{|c|}{\textbf{74.8}}&\multicolumn{1}{|c|}{\textbf{79.6}}&\multicolumn{1}{|c|}{\textbf{75.8}}&\multicolumn{1}{|c|}{61.0}&\multicolumn{1}{|c|}{\textbf{67.6}}&\multicolumn{1}{|c|}{\textbf{79.6}}&\multicolumn{1}{|c|}{\textbf{74.2}}&\multicolumn{1}{|c|}{\textbf{59.7}}&\multicolumn{1}{|c|}{\textbf{66.2}}\\ \hline

\multicolumn{1}{|c|}{Improvement}&\multicolumn{1}{|c|}{158.1}&\multicolumn{1}{|c|}{303.4}&\multicolumn{1}{|c|}{-21.1}&\multicolumn{1}{|c|}{131.6}&\multicolumn{1}{|c|}{182.3}&\multicolumn{1}{|c|}{395.4}&\multicolumn{1}{|c|}{-2.7}&\multicolumn{1}{|c|}{185.2}&\multicolumn{1}{|c|}{189.5}&\multicolumn{1}{|c|}{422.5}&\multicolumn{1}{|c|}{1.2}&\multicolumn{1}{|c|}{199.5}\\ \hline

\end{tabular}
}
\vspace{-0.2cm}
\end{table}


==> evaluation_improvement2.tex <==


\begin{table}[h]
\label{tab:gen_config_result_table}
\centering
\scalebox{0.75}{
\begin{tabular}{c|llllllllllll|}



\multicolumn{13}{c}{{\cellcolor[gray]{0.9}\textbf{Results of Generating Java Configuration for Google Checkstyle Style Guide.}}} \\
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{c|}{Rule Name-Level Metrics (\%)} &
\multicolumn{4}{c|}{Option Name-Level Metrics (\%)} &
\multicolumn{4}{c}{Option Value-Level Metrics (\%)} \\
\cline{2-13} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} \\ \hline



\multicolumn{1}{c|}{Closed-book}&\multicolumn{1}{|c}{38.2}&\multicolumn{1}{c}{\underline{39.4}}&\multicolumn{1}{c}{58.6}&\multicolumn{1}{c}{\underline{47.1}}&\multicolumn{1}{|c}{20.6}&\multicolumn{1}{c}{24.0}&\multicolumn{1}{c}{35.7}&\multicolumn{1}{c}{28.7}&\multicolumn{1}{|c}{33.8}&\multicolumn{1}{c}{\underline{28.8}}&\multicolumn{1}{c}{42.9}&\multicolumn{1}{c}{\underline{34.5}}\\ \hline

\multicolumn{1}{c|}{Name}&\multicolumn{1}{|c}{42.6}&\multicolumn{1}{c}{17.1}&\multicolumn{1}{c}{81.2}&\multicolumn{1}{c}{28.3}&\multicolumn{1}{|c}{23.5}&\multicolumn{1}{c}{11.3}&\multicolumn{1}{c}{53.6}&\multicolumn{1}{c}{18.7}&\multicolumn{1}{|c}{33.8}&\multicolumn{1}{c}{12.5}&\multicolumn{1}{c}{59.4}&\multicolumn{1}{c}{20.7}\\ \hline

\multicolumn{1}{c|}{ND}&\multicolumn{1}{|c}{44.1}&\multicolumn{1}{c}{25.7}&\multicolumn{1}{c}{80.9}&\multicolumn{1}{c}{39.0}&\multicolumn{1}{|c}{29.4}&\multicolumn{1}{c}{20.1}&\multicolumn{1}{c}{63.2}&\multicolumn{1}{c}{30.5}&\multicolumn{1}{|c}{30.9}&\multicolumn{1}{c}{17.3}&\multicolumn{1}{c}{54.4}&\multicolumn{1}{c}{26.2}\\ \hline

\multicolumn{1}{c|}{NDO}&\multicolumn{1}{|c}{\underline{51.5}}&\multicolumn{1}{c}{23.4}&\multicolumn{1}{c}{\textbf{\underline{84.1}}}&\multicolumn{1}{c}{36.6}&\multicolumn{1}{|c}{\underline{51.5}}&\multicolumn{1}{c}{23.0}&\multicolumn{1}{c}{\textbf{\underline{82.6}}}&\multicolumn{1}{c}{36.0}&\multicolumn{1}{|c}{\underline{39.7}}&\multicolumn{1}{c}{17.7}&\multicolumn{1}{c}{\underline{63.8}}&\multicolumn{1}{c}{27.8}\\ \hline

\multicolumn{1}{c|}{ND (RAG)}&\multicolumn{1}{|c}{16.2}&\multicolumn{1}{c}{23.5}&\multicolumn{1}{c}{77.6}&\multicolumn{1}{c}{36.1}&\multicolumn{1}{|c}{14.7}&\multicolumn{1}{c}{20.4}&\multicolumn{1}{c}{67.2}&\multicolumn{1}{c}{31.2}&\multicolumn{1}{|c}{13.2}&\multicolumn{1}{c}{16.3}&\multicolumn{1}{c}{53.7}&\multicolumn{1}{c}{25.0}\\ \hline

\multicolumn{1}{c|}{NDO (RAG)}&\multicolumn{1}{|c}{25.0}&\multicolumn{1}{c}{31.8}&\multicolumn{1}{c}{79.4}&\multicolumn{1}{c}{45.4}&\multicolumn{1}{|c}{25.0}&\multicolumn{1}{c}{\underline{31.8}}&\multicolumn{1}{c}{79.4}&\multicolumn{1}{c}{\underline{45.4}}&\multicolumn{1}{|c}{13.2}&\multicolumn{1}{c}{17.6}&\multicolumn{1}{c}{44.1}&\multicolumn{1}{c}{25.2}\\ \hline

\multicolumn{1}{c|}{\textbf{Our Method}}&\multicolumn{1}{|c}{\textbf{81.2}}&\multicolumn{1}{c}{\textbf{92.1}}&\multicolumn{1}{c}{\textbf{\underline{84.1}}}&\multicolumn{1}{c}{\textbf{87.9}}&\multicolumn{1}{|c}{\textbf{78.3}}&\multicolumn{1}{c}{\textbf{84.1}}&\multicolumn{1}{c}{76.8}&\multicolumn{1}{c}{\textbf{80.3}}&\multicolumn{1}{|c}{\textbf{76.8}}&\multicolumn{1}{c}{\textbf{76.2}}&\multicolumn{1}{c}{\textbf{69.6}}&\multicolumn{1}{c}{\textbf{72.7}}\\ \hline

\multicolumn{1}{c|}{Improvement (\%)}&\multicolumn{1}{|c}{57.7}&\multicolumn{1}{c}{133.8}&\multicolumn{1}{c}{0.0}&\multicolumn{1}{c}{86.6}&\multicolumn{1}{|c}{52.0}&\multicolumn{1}{c}{164.5}&\multicolumn{1}{c}{-7.0}&\multicolumn{1}{c}{76.9}&\multicolumn{1}{|c}{93.5}&\multicolumn{1}{c}{164.6}&\multicolumn{1}{c}{9.1}&\multicolumn{1}{c}{110.7}\\ \hline



\multicolumn{13}{c}{{\cellcolor[gray]{0.9}\textbf{Results of Generating JavaScript Configuration for Google ESLint Style Guide.}}} \\
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{c|}{Rule Name-Level Metrics (\%)} &
\multicolumn{4}{c|}{Option Name-Level Metrics (\%)} &
\multicolumn{4}{c}{Option Value-Level Metrics (\%)} \\
\cline{2-13} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} \\ \hline



\multicolumn{1}{c|}{Closed-book}&\multicolumn{1}{|c}{27.5}&\multicolumn{1}{c}{15.5}&\multicolumn{1}{c}{65.1}&\multicolumn{1}{c}{25.1}&\multicolumn{1}{|c}{24.8}&\multicolumn{1}{c}{11.8}&\multicolumn{1}{c}{49.4}&\multicolumn{1}{c}{19.0}&\multicolumn{1}{|c}{24.8}&\multicolumn{1}{c}{10.1}&\multicolumn{1}{c}{42.2}&\multicolumn{1}{c}{16.2}\\ \hline

\multicolumn{1}{c|}{Name}&\multicolumn{1}{|c}{18.8}&\multicolumn{1}{c}{10.5}&\multicolumn{1}{c}{83.1}&\multicolumn{1}{c}{18.6}&\multicolumn{1}{|c}{16.1}&\multicolumn{1}{c}{7.6}&\multicolumn{1}{c}{60.2}&\multicolumn{1}{c}{13.5}&\multicolumn{1}{|c}{16.1}&\multicolumn{1}{c}{7.0}&\multicolumn{1}{c}{55.4}&\multicolumn{1}{c}{12.4}\\ \hline

\multicolumn{1}{c|}{ND}&\multicolumn{1}{|c}{\underline{32.2}}&\multicolumn{1}{c}{\underline{20.8}}&\multicolumn{1}{c}{72.3}&\multicolumn{1}{c}{\underline{32.3}}&\multicolumn{1}{|c}{\underline{28.2}}&\multicolumn{1}{c}{\underline{15.3}}&\multicolumn{1}{c}{53.0}&\multicolumn{1}{c}{\underline{23.7}}&\multicolumn{1}{|c}{\underline{27.5}}&\multicolumn{1}{c}{\underline{14.2}}&\multicolumn{1}{c}{49.4}&\multicolumn{1}{c}{\underline{22.1}}\\ \hline

\multicolumn{1}{c|}{NDO}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}\\ \hline

\multicolumn{1}{c|}{ND (RAG)}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{9.2}&\multicolumn{1}{c}{79.5}&\multicolumn{1}{c}{16.5}&\multicolumn{1}{|c}{10.7}&\multicolumn{1}{c}{6.4}&\multicolumn{1}{c}{55.4}&\multicolumn{1}{c}{11.5}&\multicolumn{1}{|c}{10.7}&\multicolumn{1}{c}{6.0}&\multicolumn{1}{c}{51.8}&\multicolumn{1}{c}{10.8}\\ \hline

\multicolumn{1}{c|}{NDO (RAG)}&\multicolumn{1}{|c}{16.8}&\multicolumn{1}{c}{7.8}&\multicolumn{1}{c}{\textbf{\underline{85.5}}}&\multicolumn{1}{c}{14.4}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{5.7}&\multicolumn{1}{c}{\textbf{\underline{62.7}}}&\multicolumn{1}{c}{10.5}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{5.4}&\multicolumn{1}{c}{\underline{59.0}}&\multicolumn{1}{c}{9.9}\\ \hline

\multicolumn{1}{c|}{\textbf{Our Method}}&\multicolumn{1}{|c}{\textbf{83.1}}&\multicolumn{1}{c}{\textbf{83.9}}&\multicolumn{1}{c}{67.5}&\multicolumn{1}{c}{\textbf{74.8}}&\multicolumn{1}{|c}{\textbf{79.6}}&\multicolumn{1}{c}{\textbf{75.8}}&\multicolumn{1}{c}{61.0}&\multicolumn{1}{c}{\textbf{67.6}}&\multicolumn{1}{|c}{\textbf{79.6}}&\multicolumn{1}{c}{\textbf{74.2}}&\multicolumn{1}{c}{\textbf{59.7}}&\multicolumn{1}{c}{\textbf{66.2}}\\ \hline

\multicolumn{1}{c|}{Improvement (\%)}&\multicolumn{1}{|c}{158.1}&\multicolumn{1}{c}{303.4}&\multicolumn{1}{c}{-21.1}&\multicolumn{1}{c}{131.6}&\multicolumn{1}{|c}{182.3}&\multicolumn{1}{c}{395.4}&\multicolumn{1}{c}{-2.7}&\multicolumn{1}{c}{185.2}&\multicolumn{1}{|c}{189.5}&\multicolumn{1}{c}{422.5}&\multicolumn{1}{c}{1.2}&\multicolumn{1}{c}{199.5}\\ \hline

\end{tabular}
}
\end{table}



==> evaluation_improvement2_newdata.tex <==


\begin{table}[h]
\label{tab:gen_config_result_table}
\centering
\scalebox{0.75}{
\begin{tabular}{c|llllllllllll|}



\multicolumn{13}{c}{{\cellcolor[gray]{0.9}\textbf{Results of Generating Java Configuration for Google Checkstyle Style Guide.}}} \\
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{c|}{Module-Level Metrics (\%)} &
\multicolumn{4}{c|}{Option Name-Level Metrics (\%)} &
\multicolumn{4}{c}{Option Value-Level Metrics (\%)} \\
\cline{2-13} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} \\ \hline



\multicolumn{1}{c|}{Closed-book}&\multicolumn{1}{|c}{38.2}&\multicolumn{1}{c}{\underline{38.5}}&\multicolumn{1}{c}{58.0}&\multicolumn{1}{c}{\underline{46.2}}&\multicolumn{1}{|c}{20.6}&\multicolumn{1}{c}{23.1}&\multicolumn{1}{c}{34.8}&\multicolumn{1}{c}{27.7}&\multicolumn{1}{|c}{33.8}&\multicolumn{1}{c}{\underline{27.9}}&\multicolumn{1}{c}{42.0}&\multicolumn{1}{c}{\underline{33.5}}\\ \hline

\multicolumn{1}{c|}{Name}&\multicolumn{1}{|c}{42.6}&\multicolumn{1}{c}{16.8}&\multicolumn{1}{c}{80.9}&\multicolumn{1}{c}{27.8}&\multicolumn{1}{|c}{23.5}&\multicolumn{1}{c}{11.0}&\multicolumn{1}{c}{52.9}&\multicolumn{1}{c}{18.2}&\multicolumn{1}{|c}{33.8}&\multicolumn{1}{c}{12.2}&\multicolumn{1}{c}{58.8}&\multicolumn{1}{c}{20.3}\\ \hline

\multicolumn{1}{c|}{ND}&\multicolumn{1}{|c}{44.1}&\multicolumn{1}{c}{25.2}&\multicolumn{1}{c}{80.6}&\multicolumn{1}{c}{38.4}&\multicolumn{1}{|c}{29.4}&\multicolumn{1}{c}{19.6}&\multicolumn{1}{c}{62.7}&\multicolumn{1}{c}{29.9}&\multicolumn{1}{|c}{30.9}&\multicolumn{1}{c}{16.8}&\multicolumn{1}{c}{53.7}&\multicolumn{1}{c}{25.6}\\ \hline

\multicolumn{1}{c|}{NDO}&\multicolumn{1}{|c}{\underline{51.5}}&\multicolumn{1}{c}{23.0}&\multicolumn{1}{c}{\textbf{\underline{83.8}}}&\multicolumn{1}{c}{36.1}&\multicolumn{1}{|c}{\underline{51.5}}&\multicolumn{1}{c}{22.6}&\multicolumn{1}{c}{\textbf{\underline{82.4}}}&\multicolumn{1}{c}{35.4}&\multicolumn{1}{|c}{\underline{39.7}}&\multicolumn{1}{c}{17.3}&\multicolumn{1}{c}{\underline{63.2}}&\multicolumn{1}{c}{27.2}\\ \hline

\multicolumn{1}{c|}{ND (RAG)}&\multicolumn{1}{|c}{16.2}&\multicolumn{1}{c}{23.1}&\multicolumn{1}{c}{77.3}&\multicolumn{1}{c}{35.5}&\multicolumn{1}{|c}{14.7}&\multicolumn{1}{c}{19.9}&\multicolumn{1}{c}{66.7}&\multicolumn{1}{c}{30.7}&\multicolumn{1}{|c}{13.2}&\multicolumn{1}{c}{15.8}&\multicolumn{1}{c}{53.0}&\multicolumn{1}{c}{24.4}\\ \hline

\multicolumn{1}{c|}{NDO (RAG)}&\multicolumn{1}{|c}{25.0}&\multicolumn{1}{c}{31.2}&\multicolumn{1}{c}{79.1}&\multicolumn{1}{c}{44.7}&\multicolumn{1}{|c}{25.0}&\multicolumn{1}{c}{\underline{31.2}}&\multicolumn{1}{c}{79.1}&\multicolumn{1}{c}{\underline{44.7}}&\multicolumn{1}{|c}{13.2}&\multicolumn{1}{c}{17.6}&\multicolumn{1}{c}{44.8}&\multicolumn{1}{c}{25.3}\\ \hline

\multicolumn{1}{c|}{\textbf{Our Method}}&\multicolumn{1}{|c}{\textbf{79.7}}&\multicolumn{1}{c}{\textbf{90.5}}&\multicolumn{1}{c}{\textbf{\underline{83.8}}}&\multicolumn{1}{c}{\textbf{87.0}}&\multicolumn{1}{|c}{\textbf{76.8}}&\multicolumn{1}{c}{\textbf{82.5}}&\multicolumn{1}{c}{76.5}&\multicolumn{1}{c}{\textbf{79.4}}&\multicolumn{1}{|c}{\textbf{75.4}}&\multicolumn{1}{c}{\textbf{74.6}}&\multicolumn{1}{c}{\textbf{69.1}}&\multicolumn{1}{c}{\textbf{71.8}}\\ \hline

\multicolumn{1}{c|}{Improvement (\%)}&\multicolumn{1}{|c}{54.8}&\multicolumn{1}{c}{135.1}&\multicolumn{1}{c}{0.0}&\multicolumn{1}{c}{88.3}&\multicolumn{1}{|c}{49.1}&\multicolumn{1}{c}{164.4}&\multicolumn{1}{c}{-7.2}&\multicolumn{1}{c}{77.6}&\multicolumn{1}{|c}{89.9}&\multicolumn{1}{c}{167.4}&\multicolumn{1}{c}{9.3}&\multicolumn{1}{c}{114.3}\\ \hline



\multicolumn{13}{c}{{\cellcolor[gray]{0.9}\textbf{Results of Generating JavaScript Configuration for Google ESLint Style Guide.}}} \\
\hline
\multirow{2}{*}{Approach} &
\multicolumn{4}{c|}{Module-Level Metrics (\%)} &
\multicolumn{4}{c|}{Option Name-Level Metrics (\%)} &
\multicolumn{4}{c}{Option Value-Level Metrics (\%)} \\
\cline{2-13} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} &
\multicolumn{1}{|c}{cs-Acc} &
\multicolumn{1}{c}{P} &
\multicolumn{1}{c}{R} &
\multicolumn{1}{c}{F} \\ \hline



\multicolumn{1}{c|}{Closed-book}&\multicolumn{1}{|c}{27.5}&\multicolumn{1}{c}{15.5}&\multicolumn{1}{c}{65.1}&\multicolumn{1}{c}{25.1}&\multicolumn{1}{|c}{24.8}&\multicolumn{1}{c}{11.8}&\multicolumn{1}{c}{49.4}&\multicolumn{1}{c}{19.0}&\multicolumn{1}{|c}{24.8}&\multicolumn{1}{c}{10.1}&\multicolumn{1}{c}{42.2}&\multicolumn{1}{c}{16.2}\\ \hline

\multicolumn{1}{c|}{Name}&\multicolumn{1}{|c}{18.8}&\multicolumn{1}{c}{10.5}&\multicolumn{1}{c}{83.1}&\multicolumn{1}{c}{18.6}&\multicolumn{1}{|c}{16.1}&\multicolumn{1}{c}{7.6}&\multicolumn{1}{c}{60.2}&\multicolumn{1}{c}{13.5}&\multicolumn{1}{|c}{16.1}&\multicolumn{1}{c}{7.0}&\multicolumn{1}{c}{55.4}&\multicolumn{1}{c}{12.4}\\ \hline

\multicolumn{1}{c|}{ND}&\multicolumn{1}{|c}{\underline{32.2}}&\multicolumn{1}{c}{\underline{20.8}}&\multicolumn{1}{c}{72.3}&\multicolumn{1}{c}{\underline{32.3}}&\multicolumn{1}{|c}{\underline{28.2}}&\multicolumn{1}{c}{\underline{15.3}}&\multicolumn{1}{c}{53.0}&\multicolumn{1}{c}{\underline{23.7}}&\multicolumn{1}{|c}{\underline{27.5}}&\multicolumn{1}{c}{\underline{14.2}}&\multicolumn{1}{c}{49.4}&\multicolumn{1}{c}{\underline{22.1}}\\ \hline

\multicolumn{1}{c|}{NDO}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{|c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}&\multicolumn{1}{c}{-}\\ \hline

\multicolumn{1}{c|}{ND (RAG)}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{9.2}&\multicolumn{1}{c}{79.5}&\multicolumn{1}{c}{16.5}&\multicolumn{1}{|c}{10.7}&\multicolumn{1}{c}{6.4}&\multicolumn{1}{c}{55.4}&\multicolumn{1}{c}{11.5}&\multicolumn{1}{|c}{10.7}&\multicolumn{1}{c}{6.0}&\multicolumn{1}{c}{51.8}&\multicolumn{1}{c}{10.8}\\ \hline

\multicolumn{1}{c|}{NDO (RAG)}&\multicolumn{1}{|c}{16.8}&\multicolumn{1}{c}{7.8}&\multicolumn{1}{c}{\textbf{\underline{85.5}}}&\multicolumn{1}{c}{14.4}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{5.7}&\multicolumn{1}{c}{\textbf{\underline{62.7}}}&\multicolumn{1}{c}{10.5}&\multicolumn{1}{|c}{13.4}&\multicolumn{1}{c}{5.4}&\multicolumn{1}{c}{\underline{59.0}}&\multicolumn{1}{c}{9.9}\\ \hline

\multicolumn{1}{c|}{\textbf{Our Method}}&\multicolumn{1}{|c}{\textbf{83.1}}&\multicolumn{1}{c}{\textbf{83.9}}&\multicolumn{1}{c}{67.5}&\multicolumn{1}{c}{\textbf{74.8}}&\multicolumn{1}{|c}{\textbf{79.6}}&\multicolumn{1}{c}{\textbf{75.8}}&\multicolumn{1}{c}{61.0}&\multicolumn{1}{c}{\textbf{67.6}}&\multicolumn{1}{|c}{\textbf{79.6}}&\multicolumn{1}{c}{\textbf{74.2}}&\multicolumn{1}{c}{\textbf{59.7}}&\multicolumn{1}{c}{\textbf{66.2}}\\ \hline

\multicolumn{1}{c|}{Improvement (\%)}&\multicolumn{1}{|c}{158.1}&\multicolumn{1}{c}{303.4}&\multicolumn{1}{c}{-21.1}&\multicolumn{1}{c}{131.6}&\multicolumn{1}{|c}{182.3}&\multicolumn{1}{c}{395.4}&\multicolumn{1}{c}{-2.7}&\multicolumn{1}{c}{185.2}&\multicolumn{1}{|c}{189.5}&\multicolumn{1}{c}{422.5}&\multicolumn{1}{c}{1.2}&\multicolumn{1}{c}{199.5}\\ \hline

\end{tabular}
}
\end{table}



==> exp_stat.tex <==
\begin{table}[h]
\label{tab:exp_stat_table}
\centering
\scalebox{0.8}{
\begin{tabular}{l|lll}
\multicolumn{2}{c|}{\cellcolor[gray]{0.9}\textbf{Programming Language}}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Java}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}JavaScript}\\ \hline

\multirow{3}{*}{Coding Standard} &
\multicolumn{1}{|c|}{\rule{0pt}{3ex}Coding Standard Name} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google Java Style Guide} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google JavaScript Style Guide}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{37.1k} &
\multicolumn{1}{c}{37.1k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Rules} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
\hline

\multirow{3}{*}{Tool Configuration} &
\multicolumn{1}{|c|}{Tool Config} &
\multicolumn{1}{c}{Checkstyle} &
\multicolumn{1}{c}{ESLint}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{8.3k} &
\multicolumn{1}{c}{24.7k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of RuleNames} &
\multicolumn{1}{c}{184} &
\multicolumn{1}{c}{291}\\
\hline

\end{tabular}
}

\end{table}


\begin{table}[h]
\label{tab:exp_stat_table}
\centering
\scalebox{0.8}{
\begin{tabular}{l|lll}
\multicolumn{2}{c|}{\cellcolor[gray]{0.9}\textbf{Programming Language}}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Java}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}JavaScript}\\ \hline
\multirow{5}{*}{Benchmark} &
\multicolumn{1}{|l|}{Coding Standard} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
% \hline
\cline{2-4} &
\multicolumn{1}{|l|}{No Configuration} &
\multicolumn{1}{c}{19} &
\multicolumn{1}{c}{89}\\

\cline{2-4} &
\multicolumn{1}{|l|}{Exist Configuration} &
\multicolumn{1}{c}{49} &
\multicolumn{1}{c}{60}\\

\cline{2-4} &
\multicolumn{1}{|l|}{Config with Only RuleName} &
\multicolumn{1}{c}{7} &
\multicolumn{1}{c}{15}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|l|}{Config with RuleName and Options} &
\multicolumn{1}{c}{42} &
\multicolumn{1}{c}{45}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|l|}{Config with Multiple Rules} &
\multicolumn{1}{c}{13} &
\multicolumn{1}{c}{16}\\
\hline

\end{tabular}
}

\end{table}

\begin{table}[h]
\label{tab:exp_stat_table}
\centering
\scalebox{0.8}{
\begin{tabular}{l|lll}
\multicolumn{2}{c|}{\cellcolor[gray]{0.9}\textbf{Programming Language}}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Java}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}JavaScript}\\ \hline

\multirow{3}{*}{Code Standard} &
\multicolumn{1}{|c|}{\rule{0pt}{3ex}Code Standard Name} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google Java Style Guide} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google JavaScript Style Guide}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{37.1k} &
\multicolumn{1}{c}{37.1k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Rules} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
\hline

\multirow{3}{*}{Tool Configuration} &
\multicolumn{1}{|c|}{Tool Config} &
\multicolumn{1}{c}{Checkstyle} &
\multicolumn{1}{c}{ESLint}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{8.3k} &
\multicolumn{1}{c}{24.7k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Modules} &
\multicolumn{1}{c}{184} &
\multicolumn{1}{c}{291}\\
\hline


\multirow{5}{*}{Benchmark} &
\multicolumn{1}{|l|}{Code Std} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
% \hline
\cline{2-4} &
\multicolumn{1}{|l|}{No Configuration} &
\multicolumn{1}{c}{19} &
\multicolumn{1}{c}{80}\\

\cline{2-4} &
\multicolumn{1}{|l|}{Exist Configuration} &
\multicolumn{1}{c}{49} &
\multicolumn{1}{c}{60}\\

\cline{2-4} &
\multicolumn{1}{|l|}{Only RuleName} &
\multicolumn{1}{c}{7} &
\multicolumn{1}{c}{15}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|l|}{RuleName with Options} &
\multicolumn{1}{c}{42} &
\multicolumn{1}{c}{45}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|l|}{Multiple Rules} &
\multicolumn{1}{c}{13} &
\multicolumn{1}{c}{16}\\
\hline

\end{tabular}
}

\end{table}


\begin{table}[h]
\label{tab:exp_stat_table}
\centering
\scalebox{0.8}{
\begin{tabular}{l|lll}
\multicolumn{2}{c|}{\cellcolor[gray]{0.9}\textbf{Programming Language}}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}Java}&
\multicolumn{1}{c}{\cellcolor[gray]{0.9}JavaScript}\\ \hline

\multirow{3}{*}{Code Standard} &
\multicolumn{1}{|c|}{\rule{0pt}{3ex}Code Standard Name} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google Java Style Guide} &
\multicolumn{1}{c}{\rule{0pt}{3ex}Google JavaScript Style Guide}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{37.1k} &
\multicolumn{1}{c}{37.1k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Rules} &
\multicolumn{1}{c}{68} &
\multicolumn{1}{c}{149}\\
\hline

\multirow{3}{*}{Tool Configuration} &
\multicolumn{1}{|c|}{Tool Config} &
\multicolumn{1}{c}{Checkstyle} &
\multicolumn{1}{c}{ESLint}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{GitHub Stars} &
\multicolumn{1}{c}{8.3k} &
\multicolumn{1}{c}{24.7k}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Number of Modules} &
\multicolumn{1}{c}{184} &
\multicolumn{1}{c}{291}\\
\hline


\multirow{5}{*}{Benchmark} &
\multicolumn{1}{|c|}{No Configuration} &
\multicolumn{1}{c}{19} &
\multicolumn{1}{c}{89}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Exist Configuration} &
\multicolumn{1}{c}{49} &
\multicolumn{1}{c}{60}\\

\cline{2-4} &
\multicolumn{1}{|c|}{Only RuleName} &
\multicolumn{1}{c}{7} &
\multicolumn{1}{c}{15}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{RuleName with Options} &
\multicolumn{1}{c}{42} &
\multicolumn{1}{c}{45}\\
% \hline

\cline{2-4} &
\multicolumn{1}{|c|}{Multiple Rules} &
\multicolumn{1}{c}{13} &
\multicolumn{1}{c}{16}\\
\hline

\end{tabular}
}

\end{table}

